HARPO: Learning to Subvert Online Behavioral Advertising

Online behavioral advertising, and the associated tracking paraphernalia, poses a real privacy threat. Unfortunately, existing privacy-enhancing tools are not always effective against online advertising and tracking. We propose Harpo, a principled learning-based approach to subvert online behavioral advertising through obfuscation. Harpo uses reinforcement learning to adaptively interleave real page visits with fake pages to distort a tracker's view of a user's browsing profile. We evaluate Harpo against real-world user profiling and ad targeting models used for online behavioral advertising. The results show that Harpo improves privacy by triggering more than 40% incorrect interest segments and 6x higher bid values. Harpo outperforms existing obfuscation tools by as much as 16x for the same overhead. Harpo is also able to achieve better stealthiness to adversarial detection than existing obfuscation tools. Harpo meaningfully advances the state-of-the-art in leveraging obfuscation to subvert online behavioral advertising

==> docs/tables/related-work-comparison.tex <==
% Preserves Privacy? Does the technique aim to improve privacy for the user?
% Preserves Utility? Does the technique aim to maintain some customization for the user?
% Stealthy? Is the technique stealthy? Can it be detected?
% Adaptive? Does the technique adapt to the user’s current browsing interests?
% Principled? Does the technique take feedback to make decisions?
% Sequential? Does the technique rely on the sequential nature of browsing history? Related to the markovian nature of browsing behavior.

\begin{table}[t]
\begin{tabular}{>{\raggedright}p{1.1in}cccc}
\hline
Technique & Adaptive & Principled & Stealthy & Overhead \\
\hline
AdNauseam \cite{URL_ADNAUSEAM} & \ding{51} & \ding{55} & \ding{55} & \ding{51} \\
TrackThis \cite{URL_TRACKTHIS} & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
Your Online Interests: Pwned! \cite{ming2014pwned} & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
AdBudgetKiller \cite{kim2018adbudgetkiller} & \ding{55} & \ding{55} & \ding{55} & \ding{55} \\
Tracking and Tricking a Profiler \cite{Degeling18bluekaiwpes} & \ding{51} & \ding{51} & \ding{55} & \ding{55} \\
Privacy Through Solidarity \cite{biega2017privacy} & \ding{51} & \ding{55} & \ding{51} & \ding{51} \\
PBooster \cite{beigi2018protectinguserprivacy} & \ding{51} & \ding{51} & \ding{55} & \ding{51} \\
\ToolX{} & \ding{51} & \ding{51} & \ding{51} & \ding{51} \\
\hline
\end{tabular}
\label{table:comparison-rw}
\caption{Comparison of the related work in obfuscation from the perspective of the user.}
\end{table}
